Theta dependence of SU(N) gauge theories in the presence of a topological term

We review results concerning the theta dependence of 4D SU(N) gauge theories and QCD, where theta is the coefficient of the CP-violating topological term in the Lagrangian. In particular, we discuss theta dependence in the large-N limit. Most results have been obtained within the lattice formulation of the theory via numerical simulations, which allow to investigate the theta dependence of the ground-state energy and the spectrum around theta=0 by determining the moments of the topological charge distribution, and their correlations with other observables. We discuss the various methods which have been employed to determine the topological susceptibility, and higher-order terms of the theta expansion. We review results at zero and finite temperature. We show that the results support the scenario obtained by general large-N scaling arguments, and in particular the Witten-Veneziano mechanism to explain the U(1)_A problem. We also compare with results obtained by other approaches, especially in the large-N limit, where the issue has been also addressed using, for example, the AdS/CFT correspondence. We discuss issues related to theta dependence in full QCD: the neutron electric dipole moment, the dependence of the topological susceptibility on the quark masses, the U(1)_A symmetry breaking at finite temperature. We also consider the 2D CP(N) model, which is an interesting theoretical laboratory to study issues related to topology. We review analytical results in the large-N limit, and numerical results within its lattice formulation. Finally, we discuss the main features of the two-point correlation function of the topological charge density.

==> cpn1.tex <==
\section{$\theta$ dependence in the two-dimensional $CP^{N-1}$ models}
\label{cpn}

\subsection{The two-dimensional $CP^{N-1}$ model 
as a theoretical laboratory}
\label{cpngen}

Issues concerning the $\theta$ dependence can also be discussed in
two-dimensional CP$^{N-1}$ models~\cite{DDL-79,Witten-79b}, whose
Lagrangian is given by
\begin{equation}
{\cal L} = {N\over 2g} \overline{D_\mu z}\, D_\mu z ,
\label{lagrangiancpn}
\end{equation}
where $z$ is a complex $N$-component scalar field subject to the constraint
$\bar{z}z=1$,
\begin{equation}
A_\mu=i\bar{z}\partial_\mu z
\label{adef}
\end{equation}
is a composite gauge field, and $D_\mu =\partial_\mu +iA_\mu$ is a covariant
derivative.  They provide an interesting theoretical laboratory. Indeed they
present several features that hold in QCD: asymptotic freedom, gauge
invariance, existence of a confining potential between non gauge invariant
states (that is eventually screened by the dynamical constituents), and
nontrivial topological structure (semiclassical instanton solutions, $\theta$
vacua). We recall that the $CP^1$ model is equivalent to the O(3) $\sigma$
model, as can be easily seen by a change of variables. Indeed, in the case
$N=2$, the action can be written in a O(3)-symmetric form by reexpressing the
$z$ field in terms of $\vec{s}=\bar{z}\vec{\sigma} z$ where $\sigma_i$ are the
Pauli matrices.


An appealing feature of 2D $CP^{N-1}$ models is the possibility of perfoming a
systematic $1/N$ expansion, keeping $g$ fixed, around the large-$N$ saddle-point
solution~\cite{DDL-79,Witten-79b,CR-92,CR-93}, unlike 4D $SU(N)$ gauge theories.
This makes these models particularly interesting, because they allow us to
also check general nonperturbative scenarios by analytic calculations, without
necessarily resorting to numerical Monte Carlo methods of their lattice
formulation.

Analogously to 4D $SU(N)$ gauge theories, one may add a $\theta$ term to the
Lagrangian, writing
\begin{equation}
{\cal L}_\theta  = {N\over 2g} \overline{D_\mu z}\, D_\mu z -
i \theta {1\over2\pi}\,\epsilon_{\mu\nu}\, \partial_\mu A_\nu,
\label{lagrangiancpntheta}
\end{equation}
where 
\begin{equation}
q(x) ={1\over2\pi}\,\epsilon_{\mu\nu}\, \partial_\mu A_\nu
= {i\over2\pi}\,\epsilon_{\mu\nu}\, \overline{D_\mu z} D_\nu z 
\label{qcpn}
\end{equation}
is the topological charge density.  Then one may study the $\theta$ dependence
of the ground state and other observables. As in 4D $SU(N)$ gauge
theory, $q(x)$ is a renormalization-group invariant operator.

\subsection{The ground-state energy}
\label{groundstate energy}

By analogy with $SU(N)$ gauge theories, the ground state energy $F(\theta)$,
defined as in Eq.~(\ref{vftheta}), depends on $\theta$.  One may define a
dimensionless function $f(\theta)$ related to the ground state energy,
\begin{equation}
f(\theta) \equiv \xi^{2} [F(\theta)-F(0)] ,
\label{fthetacpn} 
\end{equation}
where $\xi \equiv \xi (\theta=0)$ is a length scale defined at $\theta=0$.
$\xi(\theta)$ can be defined from the second moment of the two-point
correlation function $G_P(x-y) = \langle {\rm Tr}\, P(x) P(0) \rangle$ of the
operator $P_{ij}(x) \equiv \bar{z}_i(x) z_j(x)$, i.e.  \footnote{The
  second-moment correlation length $\xi$ of $G_P(x)$ turns out to be more
  suitable for a $1/N$-expansion than the length scale $\xi_w$ (inverse mass
  gap) determined from the large-distance exponential decay of $G_P(x)$, i.e.
  $G_P(x)\sim e^{-|x|/\xi_w}$ at large $|x|$, due to its analytical properties
  in $1/N$~\cite{CR-91,CR-92}.  While using $\xi$ leads to an expansion in
  powers of $1/N$, the use of $\xi_w$ gives rise to nontrivial power
  corrections: Indeed, in the large-$N$ limit $\xi/\xi_w=\sqrt{2/3} +
  O(N^{-2/3})$.  }
\begin{equation}
\xi(\theta)^2 \equiv { \int d^2 x \;{1\over 4} x^2 G_P(x)\over  \int d^2 x  \;G_P(x) }.
\label{xidefcpn}
\end{equation}
The scaling function $f(\theta)$ can be expanded around $\theta=0$ as
\begin{equation}
f(\theta) = {1\over 2} C \theta^2 \left( 1 + \sum_{n=1} b_{2n} \theta^{2n} \right) ,
\label{fthetacpnexp} 
\end{equation}
where $C$ is the dimensionless quantity $\chi\xi^2$ at $\theta=0$, and $\chi$
is the topological susceptibility
\begin{equation}
\chi = \int d^2 x \langle q(0) q(x) \rangle .
\label{chicpn}
\end{equation}


\subsection{$\theta$ dependence in the large-$N$ limit}
\label{thetadepcpnln}


The $\theta$ dependence of the theory can be investigated within the $1/N$
expansion.  In the large-$N$ limit we
have~\cite{luescher-78,DDL-79,Witten-79b,CR-91}
\begin{equation}
f(\theta) = {1\over 4\pi N}  \theta^2  + O(1/N^2)
\label{thetadepcpn}
\end{equation}
for $|\theta|<\pi$, thus the topological susceptibility is $O(1/N)$,
\begin{equation}
C = {\partial^2 f(\theta)\over d \theta^2}\Bigg|_{\theta{=}0} 
= \chi\xi^2 = {1\over 2\pi N} + O(1/N^2).
\label{chim2largen}
\end{equation} 
As with 4D $SU(N)$ gauge theories (see Sec.~\ref{largeNsec} and in particular
Eqs.~(\ref{conj1}) and~(\ref{conj2})), the $2\pi$ periodicity of the $\theta$
dependence must give rise to a cusp at $\theta=\pi$, and therefore to a
singular behavior, which will be further discussed in Sec.~\ref{thetapi}.

The coefficients $b_{2n}$ of the expansion (\ref{fthetacpnexp}) are obtained
from appropriate $2n$-point correlation functions of the topological charge
density operators at $\theta=0$.  The analysis of the $1/N$-expansion Feynman
diagrams~\cite{CR-92} of the connected correlations necessary to compute
$b_{2n}$ shows that they are suppressed in the large-$N$ limit,
as~\cite{DMPSV-06}
\begin{equation}
b_{2n} = O(1/N^{2n}).
\end{equation}
Rather cumbersome calculations lead to the results~\cite{DMPSV-06} 
\begin{eqnarray}
b_2= -{27\over 5 N^2}+ O(1/N^3), \qquad
b_4= -{1830\over 7 N^4}+ O(1/N^5). 
\end{eqnarray} 

The above results are consistent with large-$N$ scaling arguments applied to
the Lagrangian (\ref{lagrangiancpn}), which indicate that the relevant
$\theta$ parameter in the large-$N$ limit should be $\bar{\theta}\equiv
\theta/N$.  This implies that the ground-state energy can be rewritten as
\begin{eqnarray} 
&&f(\theta) = N \bar{f}(\bar{\theta}\equiv \theta/N), 
\label{fthetabarcpn}\\ 
&& \bar{f}(\bar{\theta}) = 
{1\over 2} \bar{C} \bar{\theta}^2 
( 1 + \sum_{n=1} \bar{b}_{2n} \bar{\theta}^{2n} ), 
\nonumber
\end{eqnarray}
where $\bar{C}\equiv N C$ and $\bar{b}_{2n}=N^{2n}b_{2n}$ are $O(N^0)$.
Note the analogy with the expected $\theta$ dependence of the ground-state
energy in 4D $SU(N)$ gauge theories, cf.  Eq.~(\ref{lnexp}).

Within the $1/N$ expansion one may also study the dependence of the mass
$M(\theta)\equiv \xi(\theta)^{-1}$
on the parameter $\theta$. We write
\begin{equation}
M(\theta) \equiv \xi(\theta)^{-1} = M\left( 1 + m_2 \theta^2 + ... \right).
\label{gmexcpn}
\end{equation} 
The analysis of the corresponding diagrams in the $1/N$ expansion indicates
that $m_2$ is suppressed as
\begin{equation}
m_2 = O(1/N^2).
\end{equation}
Once again, the relevant parameter is seen to be $\bar{\theta}\equiv
\theta/N$.


Concerning the relevance of semiclassical instanton solutions in the context
of the $1/N$ expansion in $CP^{N-1}$ models, it was shown in
Ref.~\cite{Jevicki-79} that, at the quantum level, instantons appear in the
form of poles of the effective action, instead of stationary points, and that
the $1/N$ expansion and the semiclassical method correspond to two alternative
contour integrations of the path integral. The problem of the summability of
the instanton contributions~\cite{FFS-79} has been discussed in
Ref.~\cite{David-84}.  The compatibility of instanton models and large-$N$
expansion has been also addressed in Refs.~\cite{DM-00,KT-08}.





\subsection{Lattice calculations at $\theta=0$}


2D $CP^{N-1}$ models have also been studied by exploiting lattice techniques,
based on the straighforward discretization of the continuum
action~\cite{DHMNP-81} (in the following we set the lattice spacing $a=1$) 
\begin{equation}
S_L = -N\beta\sum_{n,\mu}\left|\bar z_{n+\mu}z_n\right|^2
\label{standard}
\end{equation}
or the lattice action~\cite{RS-81,DHMNP-81,BL-81}:
\begin{equation}
S_\lambda = -N\beta\sum_{n,\mu}\left( 
   \bar z_{n+\mu}z_n\lambda_{n,\mu} +
   \bar z_nz_{n+\mu}\bar\lambda_{n,\mu} - 2\right),
\label{basic}
\end{equation}
where $\beta=1/g$, $z_n$ is a complex $N$-component vector, constrained by the
condition $\bar z_nz_n = 1$, and $\lambda_{n,\mu}$ is an auxiliary $U(1)$ variable.
The lattice $CP^{N-1}$ model represents a very useful theoretical laboratory for
testing the various numerical methods to determine topological
properties, and in particular the topological susceptibility, also because the
results can be compared with the analytic large-$N$ calculations.

A lattice topological charge density operator $q_L$, having the correct
classical continuum limit $q^L(x) = a^2 q(x) + O(a^4)$, can be defined as
\begin{equation}
q_L(x) = -{i\over 2\pi}\sum_{\mu\nu} \epsilon_{\mu\nu}
   {\rm Tr}\left[ P(x)\Delta_\mu^{\rm s} P(x) 
   \Delta_\nu^{\rm s} P(x) \right],
\label{localq}
\end{equation}
where $\Delta^{\rm s}$ is a symmetrized version of the finite derivative:
$\Delta^{\rm s}_\mu P(x) = {1\over 2} [P(x{+}\mu) - P(x{-}\mu)]$,
and $P_{ij}(x)\equiv \bar{z}_i(x) z_j(x)$. Then, one may define the
corresponding lattice susceptibility $\chi_L=\langle \sum_x q_L(0) q_L(x)
\rangle$.  Analogously to the 4D $SU(N)$ gauge theories, see
Sec.~\ref{chilren}, the relation with the continuum topological susceptibility
is given by
\begin{equation}
\chi_{L} = a^2 Z_L^2\chi+B,
\label{chileqcpn}
\end{equation}
i.e. it involves a multiplicative renormalization and a background term which
eventually becomes dominant in the continuum limit.  
Some perturbative calculations can be found in
Refs.~\cite{FP-93,DFPV-92}.

\begin{figure}
\centerline{\psfig{width=9truecm,angle=0,file=chicpn.eps}}
\caption{ MC results for the scaling ratio $\chi\xi^2$ versus $1/N$.  Results
  indicated by crosses are taken from Ref.~\cite{DMV-04} ($N=10,15,21$,
  obtained by the geometrical method), by a circle from
  Ref.~\cite{v-93} 
  ($N=41$, geometrical method), by a box from Ref.~\cite{CRV-92-2} ($N=4$,
  heating), by a downward pointing triangle from Ref.~\cite{Burkhalter-96} ($N=4$, obtained
  using also~\cite{CRV-92-2} $\xi/\xi_w=0.985(4)$ where $\xi_w$ is the length
  scale extracted from the exponential long-distance behavior of the $P_{ij}$
  correlation function), by a right triangle from Ref.~\cite{ACDP-00} ($N=10$,
  heating) and by a left triangle from Ref.~\cite{ACDP-00} ($N=10$, cooling).
  The line shows the asymptotic large-$N$ behavior $\chi\xi^2 = 1/(2\pi N)$.
  In some cases the data are slightly shifted along the $x$-axis to make them
  visible.}
\label{chicpnfig}
\end{figure}



One can also define the topological charge by a geometrical approach.  The
original geometrical construction for the topological charge proposed in
Ref.~\cite{BL-81} is
\begin{eqnarray}
Q_g&=&\sum_n q_{n},\nonumber \\
q_{n}&=& 
{1\over 2 \pi} 
{\rm Im}\left[ \ln{\rm Tr}(P_{n+\mu+\nu}
P_{n+\mu}P_n)+ \ln{\rm Tr}
(P_{n+\nu}P_{n+\mu+\nu}P_n)\right],
\qquad \mu \neq \nu, 
\label{qgeomP}
\end{eqnarray}
where the imaginary part of the logarithm is to be taken in the interval $(-\pi, \pi)$.
For the lattice formulation (\ref{basic}) an alternative geometrical
definition $Q_{g,\lambda}$ can be given in terms of the ``gauge'' field
$\lambda_{n,\mu}$~\cite{CRV-92}. Introducing the plaquette operator
\begin{equation}
 u_{\lambda,n} =  \lambda_{n,\hat{1}} \, \lambda_{n+\hat{1},\hat{2}} 
\bar{\lambda}_{n+\hat{2},\hat{1}} \bar{\lambda}_{n,\hat{2}}, 
\label{uqt}
\end{equation}
one defines $Q_{g,\lambda}=\sum_n q_{\lambda,n}$ where $u_{\lambda,n} = \exp(i
2 \pi q_{\lambda,n})$ and $q_{\lambda,n}\in (-1/2,1/2)$.  On a finite volume
and for periodic boundary conditions $q_{n}$ and $q_{\lambda,n}$ generate
integer values of the total topological charge for each configuration.  They
are not analytical functions of the lattice fields $z$ and $\lambda$, and fail
to be defined on certain ``exceptional'' configurations, which constitute a
set of measure zero.

Fermionic constructions of the lattice topological charge density, based on
overlap Dirac operator, have been considered in Refs.~\cite{ALT-05,LT-07}.

The topological properties of 2D $CP^{N-1}$ models have been investigated by a
large number of studies exploiting lattice techniques, see
Refs.~\cite{Berg-81,MPV-82,Seiberg-84,BP-85,Wolff-92,IM-92,JW-92,CRV-92,CRV-92-2,%%
HM-93,v-93,DFP-95,BBHN-96,Burkhalter-96,DFP-97,RRV-97,PS-97-2,PS-97,v-99,ACDP-00,%%
BISY-01,ADGL-03,DMV-04,BPRW-05,LT-07,KT-08}. 
A wide range of values of $N$ has been considered, both small and large, in
order to test large-$N$ calculations.  The present state of art is briefly
summarized in the following.


Many numerical works, see
Refs.~\cite{Berg-81,MPV-82,BP-85,DFPV-92,CRV-92,FP-94,DFP-95,BBHN-96,DFP-97}
have been dedicated to the $N=2$ case, which also corresponds to the $O(3)$
nonlinear $\sigma$ model. The most recent simulations using the so-called
classical perfect action~\cite{BBHN-96,DFP-97} favor what is suggested by
semiclassical arguments, that is that $\chi$ would not be a physical quantity
for this model, in that a nonremovable ultraviolet divergence affects the
instanton size distribution. The manifestation of this property on the lattice
would be that lattice estimators of $\chi$ do not properly scale approaching
the continuum limit.

This problem should not affect the topological properties of $CP^{N-1}$ models
for $N>2$.  Monte Carlo results can be found in
Refs.~\cite{PL-83,JW-92,Wolff-92,HM-92,CRV-92,CRV-92-2,HM-93,v-93,Burkhalter-96,%%
RRV-97,ACDP-00,DMV-04,ALT-05}.
They have been obtained using the various methods discussed in
Sec.~\ref{bosmeth}.  In particular, at larger $N$, say $N\gtrsim 10$, the
geometrical estimator (\ref{qgeomP}) shows scaling already at reasonable
values of the correlation length~\cite{CRV-92-2,v-93,DMV-04}.  Some results
for the dimensionless quantity $\chi\xi^2$ at $N\ge 4$ are shown in
Fig.~\ref{chicpnfig}. For $N=10$, there are accurate estimates of the
continuum limit of $\chi\xi^2$ by different
methods: $\chi\xi^2=0.0175(3)$ using the geometrical method~\cite{DMV-04},
$\chi\xi^2=0.0169(7)$ and $\chi\xi^2=0.0169(4)$ using respectively heating and
cooling~\cite{ACDP-00}, which are in good agreement.  The results clearly
approach the large-$N$ asymptotic behavior (\ref{chim2largen}).  Deviations
from this behavior are seen to be quite small, and clearly
suppressed at large $N$.  Writing 
\begin{equation}
\chi\xi^2 = {1\over 2\pi N} + {e_2\over N^2} + O(1/N^3),
\label{o1n2chi}
\end{equation}
the MC results suggest a small $O(1/N^2)$ coefficient:  $e_2\approx
0.15$.  This number can be compared with the rather cumbersome $O(1/N^2)$
calculation in the framework of the large-$N$ expansion~\cite{CR-91}, which
confirms that the $O(1/N^2)$ correction is small, but gives the number
$e_2\approx -0.060$.  The origin of this apparent discrepancy remains unclear.

Numerical MC investigations of topological charge structure in 2D $CP^{N-1}$
models are reported in Refs.~\cite{ALT-05,LT-07,KT-08}, finding evidence of
extended coherent structures, such as instantons and domain walls, which led
to a qualitative picture of the relevant vacuum structures, and how they
change with increasing $N$: from an instanton dominated vacuum at small values
of $N$, to a domain wall dominated vacuum at large $N$.



\subsection{Results around $\theta=\pi$}
\label{thetapi}

The $\theta$ dependence of $CP^{N-1}$ models, and in particular around $\theta=\pi$,
is physically relevant in condensed matter physics.  The $CP^1$ or O(3)
$\sigma$ model at $\theta=\pi$ should describe the antiferromagnetic spin 1/2
chain~\cite{Haldane-83,Affleck-89}, which is gapless.  Thus the mass gap in
the 2D O(3) $\sigma$ model is expected to vanish when $\theta\to
\pi$~\cite{AH-87,AGSZ-89,Affleck-91}.  The spectrum around $\theta=\pi$ has
been studied in Ref.~\cite{CM-04}.  The behavior of $CP^{N-1}$ models around
$\theta=\pi$ has also been discussed in connection with the theory of the
quantum Hall effect, see e.g. Ref.~\cite{PB-05} and references therein. It has
been conjectured~\cite{Affleck-88,Affleck-91} that the ground-state energy
$F(\theta)$ of $CP^{N-1}$ models with $N>2$ presents a discontinuity at
$\theta=\pi$, like the large-$N$ limit~\cite{Seiberg-84}.  We also mention the
quite general scenario argued in Ref.~\cite{AGL-03}: assuming a nontrivial
$\theta$ dependence and quantization of the topological charge, the theory
either breaks spontaneously CP at $\theta=\pi$ or shows a singular behavior at
some critical $\theta_c$ between 0 and $\pi$.

Several lattice studies have also investigated the behavior of the theory at
finite $\theta$ and not only around $\theta=0$, see
e.g. Refs.~\cite{Seiberg-84,OS-94,BPW-95,PS-97,PS-97-2,%%
BISY-01,ADGL-02,ADGL-04,BPRW-05,AGL-07,AP-07,KT-08}.
Like 4D $SU(N)$ gauge theories, the Euclidean action with the $\theta$ term is
complex, which impedes a Monte Carlo simulation of the theory using its
straightforward discretization, i.e. by adding the $\theta$ term to the lattice
formulations (\ref{standard}) or (\ref{basic}).  Essentially two approaches
have been pursued.  In one of them the topological charge distribution is
determined at $\theta=0$ by Monte Carlo simulations, and then it is used to
estimate quantities at finite $\theta$.  In an alternative approach one
gets information of the finite-$\theta$ behavior by performing Monte Carlo
simulations at complex values of $\theta$ where the action is real, and then
somehow extending the results to real $\theta$ values.  The numerical
studies~\cite{BPW-95,AGL-07,AP-07} of the critical behavior of the $CP^1$ or O(3)
$\sigma$ model have confirmed the theoretical expectation of a gapless theory
at $\theta=\pi$.  Results for $CP^{N-1}$ models with larger values of $N$, see
Refs.~\cite{BPRW-05,ADGL-04,BISY-01,PS-97,Seiberg-84}, confirm a smooth
$\theta$ dependence up to $\theta=\pi$, where there is a singularity, like
the one found in the large-$N$ limit.  In particular, in Ref.~\cite{BPRW-05} the
sign problem was overcome by simulating an appropriate $SU(N)$ quantum spin
ladder equivalent to a $CP^{N-1}$ model with $\theta=\pi$; the results provided
evidence of a first-order transition at $\theta=\pi$ (discontinuity in
the ground-state energy $F(\theta)$) with spontaneous breaking of charge
conjugation symmetry for $CP^{N-1}$ models with $N>2$.
Ref.~\cite{KT-08} used fractionally charged Wilson loops 
to infer properties related to the $\theta$ dependence, 
providing further support to the first-order transition scenario
at $\theta=\pi$ for sufficiently large values of $N$.



